Quantum nonlocality: How does nature do it?

In a recent note, Hance and Hossenfelder (arXiv:2211.01331) recall that "locally causal completions of quantum mechanics are possible, if they violate the assumption [called statistical independence or measurement independence] that the hidden variables do not in any way depend on measurement settings" and that, consequently, the experimental violations of Bell inequalities "show that maintaining local causality requires violating statistical independence". However, Hance and Hossenfelder also argue that "we should (...) look for independent experimental evidence that can distinguish the two different options: non-locality and statistical independence, or locality and violations of statistical independence" and that "the unwillingness to consider theories without statistical independence may be the reason we do not yet have a locally causal theory for the foundations of physics that is consistent with general relativity". Here, we recall that there is a third option, namely, rejecting that measurement outcomes are governed in any way by hidden variables. Moreover, we argue that some recent results in the search for principles singling out the sets of quantum correlations for Bell and Kochen-Specker contextuality scenarios point out that this third option is scientifically more plausible and answers the question of why and how nature produces quantum nonlocality.

==> 2022-11-07_Mateus.tex <==
----

Hi Adán,

I found two typos, "complection" and "had-oc".

As for the content, I think you're taking them way too seriously. They
claim to want evidence that would support or reject statistical
independence. That's ridiculous. A violation of statistical independence
can explain away any data whatsoever.

I also think you're missing the point. The whole question is about
locality, which you do not address. How does rejecting hidden variables
and preserving measurement independence help you? It's still nonlocal.

As for the technical part, that you need ad-hoc fine-tuning to recover
the Tsirelson bound, you're entirely correct. It's a fundamental problem
for them, that they refuse to address. They can reproduce any
correlations whatsoever, there's nothing singling out quantum mechanics.
I did challenge Hossenfelder once about this. First she didn't know what
the Tsirelson bound was, after I explained to her she said it was
irrelevant. I was very surprised and asked her if her model would
violate the Tsirelson bound. She refused to answer despite my insistence.

Best,

Mateus

-----

Hi Mateus,

Thank you for being alive (and answering my questions).

I will digest your PT and FN wisdom for tomorrow.

Let me focus now on the following paragraph you wrote:

> I also think you're missing the point. The whole question is about locality, which you do not address. How does rejecting hidden variables and preserving measurement independence help you? It's still nonlocal.

Here is where Sabine and you seem to agree but I disagree. I see the following options:

(i) Preserving local hidden variables and rejecting measurement independence.

(ii) Accepting nonlocal hidden variables and keeping measurement independence.

(iii) Mixtures of (i) and (ii).

(iv) Rejecting the possibility that (any kind of) hidden variables (local or nonlocal) may play a (significant-dynamical) role in the generation of measurement outcomes, but preserving the assumption of measurement independence (this assumption plays a role in the derivation of the quantum bounds for ideal measurements). 

Notice that (iv) is not (ii). (ii) gives the local hidden variables a role in generating the measurement outcomes that (iv) denies. As a consequence, (ii) entails an ontological burden (together with the need of a fine tuning) that (iv) does not have.

Btw, Bohmian mechanics with observers with free would be an example of (ii), but without free will would be an example of (iii).

Where would MMWI (Mateus' many worlds interpretation) be?

Were you in Vienna when the Nobel madness happened?

Best,

Adán

-----

What I'm claiming is that without hidden variables you still have nonlocality. It's a simple theorem to prove that quantum mechanics violates local causality. It's in Bell's 1976 paper.

The MWI view is of course rejecting hidden variables and keeping measurement independence. Bell's proof fails because it assumes that measurements have a single outcome.

I just gave a talk about this in Vaidman's conference on Many-Worlds a couple of weeks ago, and nobody complained, so I can safely assume that this is the standard Many-Worlds point of view.

Best,

Mateus

-----

Hi Mateus,

> What I'm claiming is that without hidden variables you still have nonlocality.

What you have is a violation of "local causality". For me, "nonlocality", just mean violation of Bell inequalities. "Local causality" is a notion invented by Bell in 1976 (and called "locality" in subsequent papers) to extend Bell's 1964 theorem of impossibility of deterministic local hidden-variable theories to
local hidden-variable theories which are not deterministic (i.e., the way the hidden variables "guide" the measurement outcomes is not deterministic). However, first, Clauser and Horne did this extension before (in 1974), but they were polite and wrote that they were considering theories which are "essentially stochastic hidden-variable theories `with a certain local character' considered by Bell [in 1971]". Second, we are still talking about a notion, local causality, that applies to local hidden-variables.

We (you and me) may be meaning different things when we say that we reject the idea that hidden variables play no significant role in the generation of measurement outcomes.

> The MWI view is of course rejecting hidden variables and keeping measurement independence. Bell's proof fails because it assumes that measurements have a single outcome.

To me, the "universal wave function" in (some versions of) the MWI is pretty much a big hidden variable (with branches in each world), which is plays a similar role that one the "quantum potential" plays in Bohmian mechanics. I am reluctant to say that the MWI is "rejecting hidden variables".

Best,

Adán

PS. A newer version of the note is attached. Thank you again for your comments.

-----


